MRZ code extraction from visa and passport documents using convolutional neural networks

Detecting and extracting information from Machine-Readable Zone (MRZ) on passports and visas is becoming increasingly important for verifying document authenticity. However, computer vision methods for performing similar tasks, such as optical character recognition (OCR), fail to extract the MRZ given digital images of passports with reasonable accuracy. We present a specially designed model based on convolutional neural networks that is able to successfully extract MRZ information from digital images of passports of arbitrary orientation and size. Our model achieved 100% MRZ detection rate and 98.36% character recognition macro-f1 score on a passport and visa dataset.

==> reply.tex <==
Reviewer 1
1. There is no comparison of presented method with other end-to-end test spotting and recognition methods. Authors not compare with well known state-of-the-art methods such as pure EAST and modification and others (authors can check ICDAR 2019 completions)
Reply: We added comparison with end-to-end text spotting methods textspotter, masktextspotter and CharNET and showed that our approach outperforms these text spotting approach by a large margin on one private dataset and two large public datasets. 

2. Experimental set-up and evaluations: datasets are closed and there
is no comparison with others on open datasets. There is no speed and
complexity evaluation for presented methods and others.
Reply: We added comparison in MIDV-500 and synthetic MRZ (Table 3 and 4) datasets and showed that our approach outperforms all other approaches by a large margin. We made speed comparison on Table 4. We added a sentence: "Taken together MRZSpotter (fine) and MRZSpotter (coarse), MRZNet has 28.9M parameters."

3. Authors present new CNN model based on new combination of well known
approaches. But all evaluation is made on dataset with unknown number
of unique samples so reader is unable to see true contribution of
authors. Authors provide more detail about dataset and method.
Reply: We evaluated on open dataset MIDV-500 and synthetic MRZ.  We provided more details of our dataset include the number of countries and for each country the number of images. We also added more details of how we annotated the data. We also added following description of the data set: "These real world images were either scanned by a scanner or taken using a smart- phone camera and uploaded to our database by our customers. It reflects the real world images we encounter on a daily basis."

4. Main drawback that proposed method evaluated only on small and private dataset with unknown samples distribution. Authors may evaluate on bigger and open datasets and add to evaluation more end-to-end methods. There is high possibility of overfitting. Author must present more information about proposed mode like number of trainable parameters, train parameters and inference speed and compare with others in this field.
Reply: We added comparison with existing approaches on two publicly available datasets (one with 3335 test samples, the other with 17113 test samples) and we show the our approach outperforms existing ones by a large margin for both of these large datasets. In our dataset, we split it into training, validation and testing set and we fine tune hyperparameters using the validation set (see Ablation study) and reports results of test set to reduce overfitting. We reported trainable parameters and inference speed (Table 5). 


Reviewer 2:

1. No evaluation of existing systems of Passport control
at border between countries; Work not done on benchmark data, making
comparison unreliable and unverifiable. The authors have done the experiments on privately collected dataset.
Reply: Existing passport control at borders in countries uses RFID readers which are both closed and proprietary. Therefore authors do not have access to them and they do not represent a fair comparison. However for fair comparison, we newly added compare against existing methods and public model like CharNet.  We also newly added compare existing public datasets for benchmarking (MIDV-500 and SyntheticMRZ) on our model showing our method is reliable and verifiable and outperforms all other approaches by a large margin.

2. The Abstract and Introduction pages are fairly well written. But at a
Passport checkpoint between two countries, the passport page with
owner details including photo are grabbed and all information of the
owner are verified by the system almost instantly. Then what is the
motivation of the present work?
Reply: In the introduction, we described our motivation of automated identity verification and identifying fraud in finance such as loan applications. 

3. I would like Fig 1a to be more focused and well visible. Fig 1b could
also show the relevant page of the passport bigger, to make easy
(human) visual identification of the MRZ region and explanation about
it.
Reply: We enlarged Fig 1 and made it more focused

4. The authors should mention if the 2 lines of text, each consisting of
44 characters is accepted as Universal standard for MRZ code.
The survey of related works are surveyed fairly well. However, the
authors should identify the lacuna of these methods, which prompted
them to conduct this work.
Reply: We added in the background that "While alternative MRZ formats are employed in documents such as ID card, we limit this work to consider only this MRZ format most commonly found in passport and visa images." In the related work - Passport MRZ detection and extraction section we described the poor MRZ detection accuracy achieved by exitsting solutions

5. The MRZnet proposed by the authors consists of coarse and fine
detection of MRZ regions followed by identification/recognition of the
2-line codes, as depicted in Fig. 2. They do image skew correction at
the beginning, so that the identified bounding box is made of
horizontal-vertical lines. The skew correction method is not described
here and the recognition method, whose basis is MobileNet V2 network,
is admittedly borrowed from a different source (Ref 17 of this paper).
The authors should provide justification of using this network, since
it is normally used in mobile environment while the MRZ region of a
Passport is imaged in static condition. The reason of doing small
modifications in the network structure and choice of loss functions
(Eq. 2 - 6) etc. in the net should also be justified.
Reply: The skew correction is handled by EAST as it report a rotation angle of the bounding box. We described why we choose MobileNet V2: "Because we use cpu to run models in production, we adopt MobileNetV2 as the backbone as it is a portable network with smaller computational cost." For loss functions, we just adopted the one adopted by EAST as described in the paper except for loss of score map which we adopted dice loss. We added a table in Ablation study (table 8) comparing the balanced cross entropy loss adopted by EAST and dice loss as adopted by our approach and showed dice loss resulted in better performance.

6 The dataset used in the current experiment is not a benchmark one.
Then how  did the authors compare their method with four others?
Also, how many 'different countries' Passport images are there in
their experimental dataset?
This question of generalization should be addressed.
Reply: We added two publicly available dataset MIDV-500 and SyntheticMRZ. We added a sentence "The dataset include 2687 passport images and 2133 visa images from 85 countries." We reported the sample size of different countries in Table 1.

7. Existing systems at border posts could be added.
Reply: We wasn't able to find any references. It is unlikely that information regarding the technology actually used by the border posts is publicly available due to security reasons.

